Interference-free Operating System: A 6 Years' Experience in Mitigating Cross-Core Interference in Linux

Real-time operating systems employ spatial and temporal isolation to guarantee predictability and schedulability of real-time systems on multi-core processors. Any unbounded and uncontrolled cross-core performance interference poses a significant threat to system time safety. However, the current Linux kernel has a number of interference issues and represents a primary source of interference. Unfortunately, existing research does not systematically and deeply explore the cross-core performance interference issue within the OS itself. This paper presents our industry practice for mitigating cross-core performance interference in Linux over the past 6 years. We have fixed dozens of interference issues in different Linux subsystems. Compared to the version without our improvements, our enhancements reduce the worst-case jitter by a factor of 8.7, resulting in a maximum 11.5x improvement over system schedulability. For the worst-case latency in the Core Flight System and the Robot Operating System 2, we achieve a 1.6x and 1.64x reduction over RT-Linux. Based on our development experience, we summarize the lessons we learned and offer our suggestions to system developers for systematically eliminating cross-core interference from the following aspects: task management, resource management, and concurrency management. Most of our modifications have been merged into Linux upstream and released in commercial distributions.

==> tex/approach.tex <==
\section{Approach Overview}
\eat{总分结构}
We realize our strategy as a framework/tool, \toolname, of which workflow is shown in Figure~\ref{fig:workflow}. The input of \toolname is \blank{}. The output of \toolname is \blank{}. \toolname has \blank{} components/steps. The first component is \blank{}, which accepts \blank{} and outputs \blank{}. Intuitively, the first component does \blank{}. We do this because \blank{}. The second component is \blank{}, which accepts \blank{} and outputs \blank{}. Intuitively, the second component does \blank{}. We do this because \blank{}. The third component is \blank{}, which accepts \blank{} and outputs \blank{}. Intuitively, the third component does \blank{}. We do this because \blank{}. 

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{fig/workflow.png}
	\caption{Your beaultiful workflow picture}
	\label{fig:workflow}
\end{figure*}
\section{Design}
In this section, we discuss the design details of the components of \toolname. 
\explain{I will make an example for one component, add more based on your need}
\subsection{Component 1}
The goal of \blank{the name of component 1} is \blank{}. We use  \blank{the name of component 1} because \blank{}. 

On the high-level, \blank{the name of component 1} is a \blank{a few sentences for high level description}. We need to address \blank{} engineering problems in component \blank{}, which are \blank{}, \blank{}, and \blank{}. 

\explain{There are some examples}
To address the engineering/technical problem \blank{}, we leverage a data structure \blank{}. This data structure is a graph whose nodes are \blank{} and edges are \blank{}. This graph is an attributed graph. Therefore, each node has an attribute that represents \blank{}. Formally, we define the graph as \blank{your mathematical equations}.

To address the engineering/technical problem \blank{}, we leverage a deep learning model \blank{}. We choose this deep learning model \blank{} because it can \blank{}. The deep learning model consists of \blank{} components, which are \blank{}. Formally, the deep learning model is \blank{your math}.We choose this deep learning model \blank{} because it can \blank{}. The deep learning model consists of \blank{} components, which are \blank{}. Formally, the deep learning model is \blank{your math}.



To address the engineering/technical problem \blank{}, we propose a heuristic algorithm. On the high level, our algorithm does \blank{}. The formal pseudocode is in Algorithm~\ref{}. Specifically, \blank{discuss the critical steps in the Algorithm}



==> tex/concurrency.tex <==
\section{Concurrency and Coordination}
\label{s:concurrency}

% \subsection{Challenges}
% \label{ss:con_ch}

On multicore processors, concurrency and synchronization are inevitable.
Especially for a single OS kernel, the synchronization between isolated and
non-isolated cores is a critical issue. The Linux kernel employs various
synchronization mechanisms that introduce different degrees and types of cross-core
interference. 


Especially when the single OS kernel is shared by isolated and non-isolated
cores, synchronization between them is required. The Linux currently employs
various synchronization mechanisms that introduce different degrees and types of
cross-core interference. We classify and examine these mechanisms and show that
each category has different interference problems.

\begin{itemize}
\item \textbf{Lock Constrains.} Lock is a common synchronization mechanism for
existing OS design. General-purpose systems focus more on the performance of
locks~\cite{mcs_lock_journal,cohort_ppopp_12}, \ziqi{while real-time systems
bound the blocking of high-priority tasks by low-priority}
ones~\cite{lock_rtas_08,spin_rtss_16}. Unfortunately, many locks in Linux do not
incorporate real-time protocols, making interference hard to avoid.
\item \textbf{Global Synchronization.} To reduce the contention on shared
variables, some synchronization methods use local variables and message
communication to achieve global consistency. Although this approach can lower
the average overhead by reducing cache contention and improving memory locality,
the all-to-all message communication can significantly increase the worst-case
execution time and cause interference.
\end{itemize}

\subsection{Lock-based Synchronization}
\label{ss:jiffes}

% \head{Background.}
Jiffies is a kernel unit to record the number of timer ticks that have elapsed
in the system. It is a globally shared variable. Therefore, accessing and
updating the jiffies requires synchronization across multiple cores. The current
implementation employs a combination of multiple methods, including disabling
interrupts and using {\tt seqlock}. \footnote{ {\tt seqlock} is an efficient
reader-writer consistency mechanism. It contains a spin lock to serialize
concurrent writers, and an atomic counter that detects a stale value obtained by
a reader and directs the reader to retry. }

%\head{Problem.}
\head{Concurrent Blocking.}
The jiffies synchronization inevitably cause interference on isolated cores.
When reading the jiffies value, the isolated core may encounter an unbounded
retry loop due to conflicting modifications from non-isolated cores. If the
isolated core is a writer, it may also be blocked by concurrent writers on
non-isolated cores. Moreover, the spin lock does not follow any real-time
locking protocol.

%\head{Solution.}
\head{Solution: Compress Critical Sections.}
Our fix mitigates the interference by reducing the critical section length,
which decreases the execution time of each individual interference and lowers
the probability of being interfered with. Inside the {\tt
tick\_do\_update\_jiffies64} function, we remove unnecessary changes of the
atomic counter when the jiffies is up to date. We also identify a part that does
not need {\tt seqlock} protection, thus reducing the time of holding a lock.

\subsection{Distributed Coordination}
\label{ss:vmstate}

We present a case of message-based coordination for statistics maintenance in the system. For instance, the system has a large number of statistics related to various aspects of virtual memory, such as memory usage, paging, and disk scheduling.
Each core maintains its local statistics as the fast path, and the system aggregates data from all the cores on demand and checks for any possible inconsistencies.
For example, the {\tt vmstat\_shepherd} function schedules work on all cores to update the virtual memory statistics.
To avoid uncontrolled interference of statistics update, we provide additional interfaces that only process statistics within a given partition and ensure that the caller is also a member of that partition.

\begin{table}[t]
   \centering
  \begin{tabular}{|l|l|}
    \hline
    Name         & Description  \\ \hline
    k\_workqueue & Repeatedly allocate kernel workqueues.  \\ \hline
    u\_thread    & Create a large number of user-level threads.  \\ \hline
    u\_fork      & Repeatedly fork an empty process to consume ASID.  \\ \hline
    nic          & Repeatedly install and uninstall an unused NIC.  \\ \hline
    timer        & Create a large amount of timers.  \\ \hline
    perf\_stat   & Run above task under {\tt perf} monitor.  \\ \hline
    clac\_pi &   Calculate $\pi$ in {\tt stress-ng} testsuite.  \\ \hline
    iomix        & Disk stressing test in {\tt stress-ng}.  \\ \hline
    fault        & Generate page faults in {\tt stress-ng}. \\ \hline
    vm           & {\tt mmap} and {\tt munmap} test in {\tt stress-ng}.  \\ \hline
    sock         & Socket stressing test in {\tt stress-ng}.  \\ \hline
  \end{tabular}
  \caption{\small Interference workload running on non-isolated cores.}
  \label{tbl:interf}
\end{table}

\subsection{Summary}
\label{ss:con_sum}

In existing Linux, it is almost impossible to completely eliminate the
synchronization interference. We can only attempt to minimize the possibility
and impact of each interference. On the one hand, many system logics are deeply
coupled with synchronization mechanisms. Modifying synchronization mechanisms
can easily cause bugs and break normal functional logics. For instance, we
encountered and addressed issues related to timer ticks, but we could not
eradicate all the interferences. Another challenge is that Linux was not
originally designed for real-time systems, and thus did not account for the
multi-core synchronization methods suitable for them. To achieve no
interference, the kernel would need a major overhaul, adopting the advanced
kernel design patterns, such as quiescence-based lock-less
microkernel~\cite{speck_rtas_15}.

\vspace{1em}
\fbox{
  \parbox{0.435\textwidth}{
    Lesson 4: We should isolate resources strictly and completely whenever possible, and avoid any task synchronization or coordination between isolated partitions.
}}

\vspace{1em}
\fbox{
  \parbox{0.435\textwidth}{
    Lesson 5: When it is difficult to achieve perfect partition and avoid synchronization, the system should be redesigned to use synchronization protocols that comply with the real-time system specifications.
}}

\vspace{1em}


==> tex/relatedwork.tex <==
\section{Related Work}



==> tex/resource.tex <==
\section{Resource Management and Sharing}
\label{s:resource}

% \subsection{Challenges}
% \label{ss:res_ch}

Resource management is a fundamental function of an operating system. It is
responsible for OS to manage diverse and complex resources, such as memory, CPU,
I/O devices, and network interfaces. The goal of resource management is to
balance the resource load, maximize the resource utilization, and guarantee the
security of resources. Instead of directly managing system resources, most
applications rely on the OS to provide management services. Therefore, improper
resource management within the system can easily result in performance
interference. We identify two main reasons that are caused by resource
management and lead to performance interference:



% One core functionality of an OS is to manage diverse and complex resources, such as memory, CPU, I/O devices, and network interfaces.
% The goal of resouce management is to guarantee the resource security, balance the resource load, and maximize the resource utilization.
% Most applications do not directly manage system resources.
% They rely on the abstractions and management services of the OS.
% Therefore, improper resource management within the system can easily result in performance interference. There are two main reasons for this:

% The majority of an OS’s work involves managing a wide variety of resources, providing resources security, load balancing, and sharing, and maximizing resource utilization. Most applications do not directly manage system resources but rely on the abstractions and management services provided by the OS. Therefore, improper resource management within the system can easily result in performance interference, and there are two main reasons for this.

\begin{itemize}
\item \textbf{Diverse Operation.} The use of resources usually has a long lifetime and diverse operations, such as creation, construction, sharing, delegation, garbage collection, and deletion.
These operations spread across the entire lifecycle of the resource, making it difficult to ensure that all operations consistently comply with isolation settings.
Particularly, since the system often allows explicit affinity settings, changing affinity at different times can cause inconsistent or even contradictory configurations, leading to unanticipated interference.
\item \textbf{Resource Sharing.} OS tends to share resources among different processes or cores to improve resource utilization, system performance, and functionality. However, unintentional resource sharing can break temporal isolation and result in unpredictability. \ziqi{write more, why sharing is complex}


% Resource sharing is the primary factor that breaks temporal isolation and results in unpredictability.
% While resource sharing is often necessary for utilization, performance, or functionality requirements, there can be unintentional resource sharing that the operating system is not aware of, leading to uncontrolled interference.
\end{itemize}

\subsection{Hardware Resource: ASID}
\label{ss:res_asid}

% \head{Background.}
% TLB caches the virtual-to-physical memory mapping of a process.
% When switching a process, OS need to flush the TLB cache to avoid stale mappings.
% However, TLB flush is expensive and adds substantial overhead to context switch.
% Address Space Identifier (ASID) is a way to reduce the overhead of TLB flush and context switch. 
% An ASID is a unique identifier assigned to each process.
% CPU can use ASID to differentiate between virtual address spaces by adding an ASID item to the TLB entry.
% In this way, OS do not have to clear all the TLB entries when switching contexts.
% It can use ASID to identify the correct mapping instead.
% As a result, ASID improves the efficiency of context switching by reducing the number of TLB flush and improving the hit rate of the TLB.
% However, the number of ASIDs supported by the processor is limited, which depends on the architecture implementation.
% For example, the ARM64 processor supports 16-bit ASIDs (65536 ASIDs in total)~\cite{armdeveloper}.
% When the number of processes created in the system exceeds the ASID limit, the kernel needs to handle ASID reuse between processes.
% Furthermore, all ASIDs are shared by all the cores, so inappropriate ASID allocation can cause subtle cross-core interference.


Address Space Identifier (ASID) is a technique to reduce the overhead of TLB flush and context switch. 
An ASID is a unique identifier assigned to each process.
CPU can use ASID to differentiate between virtual address spaces by adding an ASID item to TLB entry.
In this way, OS can use ASID to identify the correct mapping and do not have to flush all the TLB entries when switching contexts. 
Existing ASID design has two constrains: indistinghuishable sharing and limited number.
For the first constrain, all ASIDs are shared by all the cores.
Thus inappropriate ASID allocation can cause subtle cross-core interference.
For the second constrain, the number of ASIDs supported by the processor is limited (e.g., ARM64 supports 16-bit, 65536 ASIDs~\cite{armdeveloper}). 
When the number of allocated ASIDs exceeds the limit, the kernel needs to handle ASID reuse between processes.


Existing ASID management follows a lazy manner. 
When a process is created, the system allocates a fresh ASID for the process. 
However, when the process exits, the system \textit{will not} release the ASID. 
After all the ASIDs are exhausted, the system reclaims and reallocates the ASID. 
Since the same ASID may have been allocated to another process, the system needs to force TLB flush.

% Here are more details about the current implementation \ziqi{in Linux?}. 
The current implementation of ASID is as follows. 
A global bitmap, \texttt{asid\_map}, is used to record the availability of each ASID.
In order to reuse and reallocation ASIDs, the system records the current version number of ASID by maintaining a global variable, \texttt{asid\_gen}.
Each process maintains a local variable, \texttt{local\_gen}, to records the \texttt{asid\_gen} at the time the process was assigned an ASID.
Upon each context switch, the process compares \texttt{asid\_gen} and \texttt{local\_gen} to judge whether the current ASID of the process has been reallocated. 
If different, it means the current ASID expires and the process needs to allocate a new ASID and flush the TLB. 
To avoid redundant TLB flush on the same core, a core-local tag is used to indicate if the core has been flushed or not.
When ASID is exhausted, the kernel clears the global \texttt{asid\_map}, increments the \texttt{asid\_gen}, and marks the TLB flush tag of all cores.
To avoid disturbing active processes, the kernel reserves ASIDs of running processes in all cores.

\begin{figure}[!t]
  \centering
  %  \vspace{-1em}
  \includegraphics[width=3.3in]{fig/asid_intr.pdf}
%  \vspace{-1em}
  \caption{\small The process of inter-core interference caused by ASID exhaustion and TLB refresh.}
  \label{fig:asid_intr}
%  \vspace{-1.5em}
\end{figure}

%\head{Problem.}
\head{Shared ASID Exhaustion.}
Existing implementation does not consider that ASID is a shared resource between
isolated and non-isolated cores.
The exhaustion of ASID in non-isolated cores is also for isolated cores, which will lead to ASID reallocation and TLB flush.
Figure~\ref{fig:asid_intr} shows the interference path of ASID exhaustion.
When the non-isolated core exhaust all ASIDs (\textcircled{1}), the system starts to flush and reallocate ASIDs (\textcircled{2}) and marks the TLB flush tag of all cores (\textcircled{3}).
When a context switch occurs in the isolated core(\textcircled{4}), the process finds its ASID expires and request a new one from \texttt{asid\_map}.
Because the ASID operations (e.g. allocation and flush) requires modifying the global variable \texttt{asid\_map} and \texttt{asid\_gen}, a spinlock is used for synchronization.
This lock can block concurrent access to \texttt{asid\_map} on the isolated core, which is an undesired interference
(\textcircled{5}).
%Similarly, accessing \texttt{asid\_map} requires the lock and can be blocked by another concurrent context switch. 
If a new ASID is allocated, the process has to flush the TlB (\textcircled{6}).
%\ziqi{which is the second expensive interference on the isolated core.} 
Moreover, after the process resumes, it suffers TLB miss when accessing memory
(\textcircled{7}).
It significantly slows down the process execution.
% and is the third source of cross-core interference.
Figure~\ref{fig:tlb_i} summarizes the interference on the isolated core.
% , so ASID allocation and flush can cause notable
% cross-core interference

\begin{figure}[!b]
  \centering
  %  \vspace{-1em}
  \includegraphics[width=3.3in]{fig/tlb.pdf}
%  \vspace{-1em}
  \caption{\small Cross-core interference of ASID management.}
  \label{fig:tlb_i}
%  \vspace{-1.5em}
\end{figure}

%\begin{figure}[!t]
%  \begin{center}
%    \vspace{-1em}
    % \begin{lstlisting}[numbers=left,numbersep=3pt,xleftmargin=2em,framexrightmargin=-0.9em,framexleftmargin=1.1em, style=eulerc,emphstyle=\color{dgray}\ttfamily,emph={[2]asid_expire,lock,unlock,wait_queue_add,wait_queue_move,wait_for_readers,flip_counter,wait_for_readers,wake_waiters,wait_sync},morekeywords={spin_lock_t, bit_map_t}, mathescape=true]
%    \lstinputlisting[language=C]{code/asid.c}
 % \end{center}
%  \caption{\small The pseudocode for the ASID management operations with ASID domain.
%  All accessed variables are either domain-wide or core-local.}
%  \label{fig:asid_code}
%  \vspace{-2em}
%\end{figure}

%\head{Solution.}
\head{Solution: ASID Isolation.}
To eliminate the cross-core interference of ASID, we propose to partition the ASID space and integrate ASID into the core isolation.
More importantly, given the predictability of real-time applications, both the number of processes they need and the rate at which they create processes are bounded.
Based on this observation, we can preserve enough ASID to the isolated cores and guarante non-isolated cores never use reserved ASIDs.
By separating the ASID allocation and management of real-time processes from non-isolated cores, we can avoid ASID interference. 
Similar idea also applies to x86 who has the same mechanism as but fewer IDs than ARM.

% , it is easy to partition the space since each ASID is a
% discrete identifier
While the ASID space is shared across all cores, we divide the ASID space into two subspaces. Isolated cores and non-isolated cores use different subspace.
Each subspace manages an independent ASID range, thus lock and generation counter are also managed separately. %(lines \blank{} - \blank{} in Figure~\ref{fig:asid_code}).
%To partition the ASID, we introduce a new abstraction called ASID domain.
%We use different ASID domains to isolate ASID space.
%Isolated cores and non-isolated cores use different domains.
%Concretely, an ASID domain includes a fixed number of ASIDs, a list of cores that share the ASID range, a bitmap to track the availability of each ASID, a lock and a generation counter (lines 1 - 7 in Figure~\ref{fig:asid_code}).
In ASID management operations, We first check whether the current core is an isolated core.
Then, all subsequent operations are restricted to corresponding subspace.
The basic process of each ASID operation are similar to the existing implementation, except that we replace global variable access with subspace-wide variables.
For example, upon a context switch, the process checks the subspace generation counter and allocates fresh ASID within its subspace.% (lines \blank{} - \blank{} in Figure~\ref{fig:asid_code}).
% Similarly, in the function {\tt asid\_flush} % (lines \blank{} - \blank{} in Figure~\ref{fig:asid_code})
Similarly, in the process of ASID flush
which is invoked after ASID exhaustion, 
%it only affects the core within the subspace.
we clear the allocation map, update the generation counter, reserve ASIDs of active processes in the subspace, and notify cores only in the subspace to flush their TLB.
%The pseudocode of our ASID management with ASID domain is listed in Figure~\ref{fig:asid_code}.
\dzm{I think code can be removed or put into appendix. The most content of code is just a repeat of the existing implementation. Seems that the process of ASID isolation is clear without code...}

With our ASID isolation approach, we can guarantee that non-isolated cores never interfere with isolated cores.
For example, if non-isolated cores exhaust ASID in their domain, they will reallocate ASID exclusively from its assigned domain.
ASIDs assigned to the isolated cores remain unaffected, and nonisolated cores will not compete for the lock with nor mark the TLB flush flag on isolated cores.

\subsection{Device Management}
\label{ss:device}

% \head{Background.}
The OS needs to clear the stale status of a device when it is updated during
plug-in, probe, or removal phases. In a general system, a device is often shared
by all the cores. Updating the device status will invoke other cores to clean up
the core-local device status. However, such cross-core processing is undesirable
in real-time systems since it triggers cross-core interferences. Particularly,
real-time applications on isolated cores explicitly avoid sharing devices with
non-isolated cores, thus there is no status that needs to be maintained on
isolated cores at all.

%\head{Problem.}
\head{Unnecessary Backlog Flushing.}
We take network interface controller (NIC) management as an example. A NIC has a per-core {\tt backlog} queue
that holds pending packets. The system needs to flush all backlog queues
periodically to prevent missing packets. For example, when uninstalling a NIC,
OS will flush all the queues, which causes interaction over all the cores.
However, the current implementation does not consider whether the flush is
necessary or not, and does not distinguish between isolated and non-isolated
cores. This causes obvious cross-core interference even when the NIC is never
used by the isolated cores.

%\head{Solution.}
\head{Solution: On-demand Flush.}
Our solution to prevent interaction from device management is to introduce a
flush operation that is triggered only when necessary. Before flushing a remote
core, we check if the target core has any pending packets. If the target core
has no pending packets, we skip the flush operation. Otherwise, we check if the
isolation status of the caller core. If the caller core is isolated, we complete
the flush operation since the flush is necessary and is not external interference.
If the caller core is not isolated, we report a warning and record the problematic
behavior.



\subsection{Summary}
\label{ss:res_sum}

Based on our development experience, we find that it is impractical to
individually investigate the usage patterns of each resource. We have devoted
considerable time to assessing the potential performance interference caused by
resources and have identified additional associated issues. For instance, when
probing a PCI device, the device specific part is distributed into different
cores regardless of core isolation. The affinity of managed interrupts cannot be
changed by users, but the kernel evenly spreads out those interrupts across all
the cores, breaking the isolation guarantee. In addition to ASID, some other
hardware resources can introduce unexpected interference via sharing. For
example, multiple cores can share tags for the last-level cache (not the cache
itself)~\cite{hisi_tags}. Such hidden sharing is pretty hard to be managed by
system designers. However, we recognize that our current approach is not
scalable. Therefore, for future system design, it is recommended to incorporate
more formal and abstract models for resource management.

\vspace{1em}
\fbox{
  \parbox{0.435\textwidth}{
    Lesson 2: Both software and hardware platforms should expose all resources to designers and users, providing them insights into the characteristics and management of the resources.
}}

\vspace{1em}
\fbox{
  \parbox{0.435\textwidth}{
    Lesson 3: Resource sharing and affinity should adhere to a formal usage contract that can be comprehensively analyzed using real-time system theory.
}}

\vspace{1em}



==> tex/task.tex <==
\section{Task Scheduling and Placement}
\label{s:design}

% \subsection{Challenges}
% \label{ss:task_ch}

Task management is the core function of an OS, which determines the task
execution, priority, and distribution. The management of tasks can significantly
affect the latency and performance for each task. Besides user tasks, the OS
also generates a significant number of tasks to perform OS functions. However,
most system tasks are opaque to users, which make it challenging for users to
analyze and control the impact. Such opaqueness can lead to unpredicted
performance interferences. Linux currently faces two severe technical challenges
for task management:


% making it challenging to analyze and control their impact, resulting in many
% unpredicted performance interferences. Linux currently faces two severe
% technical issues with task management.

\begin{itemize}
\item \textbf{Lack of Unified Isolation Model.} The system has diverse task
models and interfaces, such as kernel threads, task queues, interrupt routines,
and callback functions. These diverse task models lack a unified isolation and
management mechanism. Consequently, some module may ignore the isolation
configuration of other system modules, thus compromise the isolation guarantee.
\item \textbf{Dynamic Migration.} Due to the dynamic migration and placement
strategies, some tasks could change the isolation configuration over time.
Especially, when there are complicated dependencies among a large number of
tasks, such as task chain, derived tasks, and forking. Task migration may not
consider all associated tasks, leading to some tasks being left on undesired
cores.
\end{itemize}

Based on these two challenges, we identified two specific scenarios that cause
performance interference for task scheduling and placement: \textit{Indistinguishable
Core Activation} and \textit{Inconsistent Task Migration}. We will discuss these
two scenarios in detail in the following sections.

\begin{figure}[!t]
  \centering
  \vspace{-1em}
  \includegraphics[width=3.3in]{fig/kwq.pdf}
%  \vspace{-1em}
  \caption{\small Cross-core interference of {\tt workqueue}.}
  \label{fig:kwq_i}
 \vspace{-1.5em}
\end{figure}

\subsection{Indistingushable Core Activation}
\label{ss:workq}

% \head{Background.}
This interference happens when {\tt workqueue} operations wake up worker threads
on all cores, including the isolated ones. The {\tt workqueue} is a lightweight
mechanism for scheduling simple kernel tasks. Each {\tt workqueue} is a queue of
work items. Each work item is a function to be executed asynchronously by
multiple worker threads. The worker threads are usually organized into a
per-core thread pool and are activated by the {\tt workqueue}'s own task
scheduling policies. The policies determine when and where to execute the work
items.

%\head{Problem.}
\head{Redundant Activation.}
Manipulations on a {\tt workqueue} are possible to trigger kernel task
executions. However, due to the lack of a unified isolation model, the {\tt
workqueue} management may interfere the isolated cores. Specifically, we
identified two problems in the {\tt workqueue} implementation in the current
Linux kernel \ziqi{version?}. First, some {\tt workqueue} operations (e.g.
\texttt{pwq\_adjust\_max\_active}) indiscriminately wake up worker threads on
all cores, including the isolated ones. Second, some irrelevant operations, such
as \texttt{alloc\_workqueue}, usually activate unnecessary worker threads, and
thus activate the isolated cores. For both cases, {\tt workqueue} core will send
an IPI (Inter-Processor Interrupt) to the isolated core to wake up a worker thread.


Core activation can cause significant interference on isolated cores. When the
isolated core receives an IPI, it will perform four operations: 1) handle the
IPI, 2) switch context to the work thread, 3) execute the work item, and 4)
switch context back to the real-time task. All the four operations consume CPU
time and introduce interfere. To handle IPI, the isolated core needs to disrupt
the real-time task, which may lead to a significant jitter. The context switch
between the real-time task and the work thread also introduces extra overhead.
Moreover, the work thread execution itself introduce additional overhead to the
isolated core. 


% Concretely, we identified two problems with the current {\tt workqueue}
% implementation. 1) Some {\tt workqueue} operations (e.g.
% \texttt{pwq\_adjust\_max\_active}) indiscriminately wake up worker threads on
% all cores, including the isolated ones. 2) Some irrelevant operations, such as
% \texttt{alloc\_workqueue}, trigger unnecessary worker thread activation. These
% problems cause significant interference on isolated cores as shown in Figure
% \ref{fig:kwq_i}. The interference has three sources. First, an IPI is sent to
% the isolated core to wake up a worker thread, which consumes CPU time to handle
% the interrupt and disrupts the real-time task. Second, executing a work item
% causes extra context switches. Third, the worker thread execution interferes
% with real-time applications on the isolated core.

%\head{Solution.}
\head{Solution: Core Activation Restriction.}
To address the above problems, we propose three technical solutions to restrict
the activation of worker threads on isolated cores. First, we only wake up a
worker thread on a core when there are work items pending on that core. For the
cores that have no work items, we do not wake up any worker threads. Second, we
restrict the activation mechanism so that a worker thread can only wake a core
within the same partition. The partition is defined by the isolation
configuration. It means that a non-isolated core can only send an IPI to another
non-isolated core but can not send an IPI to an isolated core. Third, we check
and guarantee that irrelevant operations (e.g. {\tt alloc\_workqueue}) do not
contain any thread activation and task distribution operation.


% restrict the activation of CPU cores to those within the same partition.
% This means that a non-isolated core will only send an IPI to another non-isolated core after checking the isolation configurations.
% Third, we ensure that irrelevant operations do not contain any thread activation and task distribution.

\subsection{Inconsistent Task Migration}
\label{ss:interrupt}

% \head{Background.}

Task migration is a common operation that can be triggered by either users or
the OS. \ziqi{Explain what is migration} The central design of a migration
policy is to determine which task to migrate and the migration destination.
Migrating a task involves various components from the kernel to user-level
tools, and any mismatch between the migration component can lead to
inconsistency and interference.

%\head{Problem.}
\head{Isolation-Agnostic Migration.} 
A typical interference case of inconsistent migration is as follows. A task is
initially placed on isolated cores due to an incorrect core selection. As the
task executes, it spawns other tasks on the same cores. When the OS or a user
detects the misplacement and try to migrate the task, the migration interface
may not apply to the spawned tasks. These spawned tasks are left on the isolated
cores, leading to interference. For instance, some 
microphone drives pins its IRQ
threads by using \texttt{cpumask\_local\_spread} function. This function returns
a core but does not check the isolation status. When the IRQ thread is later
moved to a non-isolated core, the spawned kernel threads remain on the isolated
core. Moreover, the user-level utility function {\tt irqbalance} also ignores the isolation
configuration of cores when there is no explicit user request.

% and then it
% spawns other tasks on the same cores. When the OS or a user detects the
% misplacement and migrates the task, the migration interface may not cover the
% spawned tasks, leaving them on the isolated cores and leading to interference.
% For instance, some MIC drives pins its IRQ threads by using
% \texttt{cpumask\_local\_spread} function. This function returns a core but does
% not check the isolation status. When the IRQ thread is later moved to a
% non-isolated core, the spawned kernel threads remain on the isolated core.
% Moreover, the user-level utility {\tt irqbalance}~\cite{irq_balance}
% \ziqi{citation} also ignores the isolation configuration of cores when there is
% no explicit user request. 
% isolated cores without an explicit request from users. \ziqi{last sentence}

%\head{Solution.}
\head{Solution: Isolation-Aware Selection.}
To include the isolation statue to the task migration, we propose two solutions
to select the target core for migration. First, for the
\texttt{cpumask\_local\_spread} function, we modify the core selection logic to
check the isolation status. We only select a core from the online non-isolated
cores. Only if all non-isolated cores are offline will we return an isolated
core. Second, for the \texttt{irqbalance} function, we check if the user
explicitly provides a core list for balancing. If not, we follow the OS default
isolation configuration that excludes the isolated cores specified in the boot
parameters.

% Our solution does not address the root cause of the migration problem, but rather handles each case separately. In \texttt{cpumask\_local\_spread}, we select a core from the intersection of online cores and non-isolated cores. Only when all non-isolated cores are offline, we return an isolated core.To fix \texttt{irqbalance}, we check if the user explicitly provides a specific core list for balancing. If not, we follow the OS default isolation configuration that excludes the isolated cores specified in boot parameters.

\subsection{Summary}

After analyzing the technical challenges and fixing specific problems in Linux task scheduling, we are particularly attentive to potential performance interference caused by various task management functions.
Following this approach, we have identified more performance interference issues in addition to the two cases explained above.
For example, when launching a kernel thread, the system only considers core isolation indicated by the {\tt isolcpus} boot parameter, and ignores {\tt nohz\_full}.
The system also selects the isolated core incorrectly when migrating user threads to idle cores.
Furthermore, the system does not consider core isolation when distributing networking packet processing tasks.
As discussed in \S\ref{s:intro}, our modifications do not lead to in a unified mechanism due to practical commercial purposes.
Therefore, our existing modifications may not resolve all issues or prevent similar ones from arising in the future.
However, we believe that interference control and isolation configuration need to be integrated into task management during future system design.

\vspace{1em}
\fbox{
  \parbox{0.435\textwidth}{
    Lesson 1: It is crucial to develop a unified spatial isolation mechanism and interface that mandates all types of tasks to apply and respect global isolation.
}}
\vspace{1em}





==> tex/threatmodel.tex <==
\section{Theat Model and Assumptions}

We follow the same threat model used in previous work~\cite{}. Specifically, we assume the OS/hardware is uncompromised. We do not consider side-channel attacks. 
